Analysing the Behaviour of Tree-Based Neural Networks in Regression Tasks

The landscape of deep learning has vastly expanded the frontiers of source code analysis, particularly through the utilization of structural representations such as Abstract Syntax Trees (ASTs). While these methodologies have demonstrated effectiveness in classification tasks, their efficacy in regression applications, such as execution time prediction from source code, remains underexplored. This paper endeavours to decode the behaviour of tree-based neural network models in the context of such regression challenges. We extend the application of established models--tree-based Convolutional Neural Networks (CNNs), Code2Vec, and Transformer-based methods--to predict the execution time of source code by parsing it to an AST. Our comparative analysis reveals that while these models are benchmarks in code representation, they exhibit limitations when tasked with regression. To address these deficiencies, we propose a novel dual-transformer approach that operates on both source code tokens and AST representations, employing cross-attention mechanisms to enhance interpretability between the two domains. Furthermore, we explore the adaptation of Graph Neural Networks (GNNs) to this tree-based problem, theorizing the inherent compatibility due to the graphical nature of ASTs. Empirical evaluations on real-world datasets showcase that our dual-transformer model outperforms all other tree-based neural networks and the GNN-based models. Moreover, our proposed dual transformer demonstrates remarkable adaptability and robust performance across diverse datasets.

==> Introduction_old.tex <==
Deep learning models, particularly those adept at handling tree-structured data, find significant applicability in the domain of source code analysis, where the source code can be represented as a tree. This is exemplified by their use in various tasks such as classification of source code~\cite{Bui2018,kanade2020,CNN_tree}, detection of code clones~\cite{Bui:21-2,Fang2020,Mehrotra2020}, identification of bugs~\cite{Hua2021,Li2021ICSE,Shi2021}, and generation of code summaries~\cite{Bui:21-1,Zhang:20,liu2021}. Central to our investigation is the neural networks' behaviour when applied to tree structures, with source code analysis serving as a prime example. It is worth noting that source code can also be represented in a textual format, thereby encapsulating the lexical content of the code~\cite{samoaaSLR2022}.
For that aim, most traditional approaches to processing source code often adopt string-based pattern matching, rule-based model transformation, and bag-of-words~\cite{ALSABBAGH2022}. However, these methods treat code fragments as plain texts, which ignore the underlying semantic information in source code, resulting in poor performance.
Source code can be represented as a tree throughout the abstract syntax tree (AST)~\cite{samoaaSLR2022}. Thus, the code can be parsed to the tree directly without prior execution. AST representation is abstract and does not include all available details, such as punctuation and delimiters. Theoretically, ASTs can be used to illustrate the syntactic structure of source code, such as the function name and the flow of the instructions (for example, in an if or while construct). Recently, some approaches combined neural networks and ASTs to constitute tree-based neural networks  (TNNs)~\cite{AST_NN}. Given a tree, TNNs learn the vector representation by recursively computing node embeddings in a bottom-up way. Popular TNN models are the Recursive Neural Network (RvNN)~\cite{DLCF}, Tree-based convolutional neural networks  (TBCNN)~\cite{CNN_tree}, and Tree-based Long Short-Term Memory (Tree-LSTM)~\cite{SDF}.
According to Samoaa et al., ~\cite{samoaaSLR2022}, source code can also be represented as a graph. The graph-structured representations can only be extracted via the intermediate representation (IR) or bytecode~\cite{Zhao2018} (e.g. control flow graphs, data flow graphs, dependency graphs, call graphs), which means that the code fragments have to be compiled successfully. However, the graphs may contribute to enriching code representations. Unfortunately, arbitrary code fragments or incomplete code snippets usually lose the import libraries or dependency packages, making the compilation fail. Such a limitation may make a large number of labelled code snippets unavailable for training, hindering the application of graph representations in practice~\cite{hua2022transformer}.
That is why, in our study, we will focus on trees as they are easier to extract, and we just need to parse the source code. 

% limitation over these approaches 
According to Samoaa~\cite{samoaaSLR2022}, the majority of the deep-learning-based approaches for source code follow the same pipeline: the approaches start with extracting lexical or syntactic features from code fragments in the form of raw text tokens, or ASTs and then use deep learning models like recurrent neural networks (RNNs) or convolutional neural networks (CNNs) to encode the tokens into vectors for downstream tasks like classification and regression.
These approaches have three major limitations: 1) RNN models inevitably suffer from the gradient vanishing problem, meaning that the gradients become vanishingly small values during model training, especially in the context of usage of AST which is very deep in most cases~\cite{mou2018tree}; 2) CNN models cannot capture the long-distance dependency information from sequential nodes of tokens in AST due to the size limitation of the sliding windows, which scan only a few nodes/tokens at a time~\cite{mou2018tree}; 3) apart from using the simplistic lexical features, the approaches for AST processing that recursively traverse entire trees from bottom to top may produce longer sequential inputs than the textual inputs, consume large amounts of computational resources and destroy the syntactical structures existing in AST~\cite{hua2022transformer}

Thus, based on the abovementioned limitations, we will use a transformer as a competitor for sequential models as well as the basis of our approach for the following reasons:
\begin{itemize}
    \item \textbf{Handling Long Dependencies:} Transformers leverage self-attention mechanisms. This allows them to weigh the importance of different parts of the input sequence directly, regardless of the distance between elements~\cite{attention}, making them well-suited for the hierarchical and complex structures of ASTs.
    \item \textbf{Parallelization:} Transformers do not process data sequentially as RNNs do. Instead, they can process entire sequences of data in parallel during training, which significantly speeds up the learning process. This is particularly advantageous when dealing with the large and intricate structures of ASTs, where computational efficiency is paramount.
    \item \textbf{Flexibility in Capturing Structural Information: }The self-attention mechanism in transformers can easily adapt to the structured nature of ASTs, capturing both the local and global context within the tree. This flexibility allows for a more nuanced understanding of code semantics compared to the fixed window size of CNNs or the sequential nature of RNNs.
    \item \textbf{Scalability:} Transformers are highly scalable and capable of handling large input sequences without significantly dropping performance. This makes them ideal for source code analysis, where ASTs can vary widely in size and complexity.
\end{itemize}

% the problem 
Another issue is that most TBNN approaches tackle a classification problem for the source code but not regression tasks. Regression tasks such as source code performance prediction (predicting the execution time for the application prior to running it) can give the developer an early indication of the runtime behaviour of their source code. Samoaa et al.~\cite{SamoaaTEPGNN} indicate that trying the TNNs approaches for regression tasks will lead to poor efficiency compared to classification tasks.  That said, these solutions are not generic enough for any source code analysis tasks. We will use the benchmark models for source code analysis to prove this claim, leading to a high classification accuracy but in a regression context. Thus, we will use code2vec~\cite{Alon19}, TBCNN~\cite{CNN_tree}, and Transformer-based networks over AST(TBAST)~\cite{hua2022transformer} as the main benchmarks for regression tasks, taking into account that we have to make some changes in the architecture of these models to fit the regression tasks. 
% @Antonio add something more about GNN.
Additionally, we explore various GNN architectures, focusing on neighbourhood information sampling and aggregation within the AST, to further enrich our analysis framework.

 
% the approach
To address all the mentioned challenges, we develop our approach based on a cross-attention dual transformer, which utilizes sequences of source code tokens and AST nodes. By employing cross-attention mechanisms between the two transformers, our model aims to elucidate the influence of individual source code tokens on AST nodes, enhancing the understanding of code semantics. 

Through this study, we will answer the following question:
\begin{itemize}
    \item \textbf{Why does the TNN behave differently in regression tasks?}
\end{itemize}   

To that aim, we analyse the behaviour of each type of architecture (convolution, sequence, and GNN) for different levels of information: node level (for every node in the AST) as in TBCNN, GNNs, and sequential transformers or path level (a path in AST, which is a sequence of nodes) as in code2vec. 
% then we use these models to encode each path into a continuous vector as a representation, then the representations for paths will be pooled together to have the final vector that represents the entire AST. 
Since we have a regression value for each source code program, we have to map each AST to the regression value. Thus, the AST has to be represented as one vector. For that aim, we will aggregate the node and path representations through the models into one continuous vector. 
To increase the reliability, we use two different real-world datasets of performance measurements. The first dataset (\emph{OSSBuild}) is real build data collected from the continuous integration systems of four open-source systems. The second (\emph{HadoopTests}) is a larger dataset which we have collected ourselves by repeatedly executing unit tests from the Hadoop open-source system in a controlled environment. 
% the results 
The results show that our dual transformer approach Outperforms both TBNN and GNN-based approaches for both datasets.  
% The conclusion sentences. 
\textcolor{red}{Add the Contribution, which is a model-centric AI for employing both code tokens and trees in the transformer based on cross attentions. Datasets that can be used by the researchers in literature.  A framework that merges all TBNN with our own model so the researchers can use this open-source framework for different tasks. }
Deep learning models, particularly those adept at handling tree-structured data, find significant applicability in the domain of source code analysis, where the source code can be represented as a tree. This is exemplified by their use in various tasks such as classification of source code~\cite{Bui2018,kanade2020,CNN_tree}, detection of code clones~\cite{Bui:21-2,Fang2020,Mehrotra2020}, identification of bugs~\cite{Hua2021,Li2021ICSE,Shi2021}, and generation of code summaries~\cite{Bui:21-1,Zhang:20,liu2021}. Central to our investigation is the neural networks' behaviour when applied to tree structures, with source code analysis serving as a prime example. It is worth noting that source code can also be represented in a textual format, thereby encapsulating the lexical content of the code~\cite{samoaaSLR2022}.
For that aim, most traditional approaches to processing source code often adopt string-based pattern matching, rule-based model transformation, and bag-of-words~\cite{ALSABBAGH2022}. However, these methods treat code fragments as plain texts, which ignore the underlying semantic information in source code, resulting in poor performance.
Source code can be represented as a tree throughout the abstract syntax tree (AST)~\cite{samoaaSLR2022}. Thus, the code can be parsed to the tree directly without prior execution. AST representation is abstract and does not include all available details, such as punctuation and delimiters. Theoretically, ASTs can be used to illustrate the syntactic structure of source code, such as the function name and the flow of the instructions (for example, in an if or while construct). Recently, some approaches combined neural networks and ASTs to constitute tree-based neural networks  (TNNs)~\cite{AST_NN}. Given a tree, TNNs learn the vector representation by recursively computing node embeddings in a bottom-up way. Popular TNN models are the Recursive Neural Network (RvNN)~\cite{DLCF}, Tree-based convolutional neural networks  (TBCNN)~\cite{CNN_tree}, and Tree-based Long Short-Term Memory (Tree-LSTM)~\cite{SDF}.
According to Samoaa et al., ~\cite{samoaaSLR2022}, source code can also be represented as a graph. The graph-structured representations can only be extracted via the intermediate representation (IR) or bytecode~\cite{Zhao2018} (e.g. control flow graphs, data flow graphs, dependency graphs, call graphs), which means that the code fragments have to be compiled successfully. However, the graphs may contribute to enriching code representations. Unfortunately, arbitrary code fragments or incomplete code snippets usually lose the import libraries or dependency packages, making the compilation fail. Such a limitation may make a large number of labelled code snippets unavailable for training, hindering the application of graph representations in practice~\cite{hua2022transformer}.
That is why, in our study, we will focus on trees as they are easier to extract, and we just need to parse the source code. 

% limitation over these approaches 
According to Samoaa~\cite{samoaaSLR2022}, the majority of the deep-learning-based approaches for source code follow the same pipeline: the approaches start with extracting lexical or syntactic features from code fragments in the form of raw text tokens, or ASTs and then use deep learning models like recurrent neural networks (RNNs) or convolutional neural networks (CNNs) to encode the tokens into vectors for downstream tasks like classification and regression.
These approaches have three major limitations: 1) RNN models inevitably suffer from the gradient vanishing problem, meaning that the gradients become vanishingly small values during model training, especially in the context of usage of AST which is very deep in most cases~\cite{mou2018tree}; 2) CNN models cannot capture the long-distance dependency information from sequential nodes of tokens in AST due to the size limitation of the sliding windows, which scan only a few nodes/tokens at a time~\cite{mou2018tree}; 3) apart from using the simplistic lexical features, the approaches for AST processing that recursively traverse entire trees from bottom to top may produce longer sequential inputs than the textual inputs, consume large amounts of computational resources and destroy the syntactical structures existing in AST~\cite{hua2022transformer}

Thus, based on the abovementioned limitations, we will use a transformer as a competitor for sequential models as well as the basis of our approach for the following reasons:
\begin{itemize}
    \item \textbf{Handling Long Dependencies:} Transformers leverage self-attention mechanisms. This allows them to weigh the importance of different parts of the input sequence directly, regardless of the distance between elements~\cite{attention}, making them well-suited for the hierarchical and complex structures of ASTs.
    \item \textbf{Parallelization:} Transformers do not process data sequentially as RNNs do. Instead, they can process entire sequences of data in parallel during training, which significantly speeds up the learning process. This is particularly advantageous when dealing with the large and intricate structures of ASTs, where computational efficiency is paramount.
    \item \textbf{Flexibility in Capturing Structural Information: }The self-attention mechanism in transformers can easily adapt to the structured nature of ASTs, capturing both the local and global context within the tree. This flexibility allows for a more nuanced understanding of code semantics compared to the fixed window size of CNNs or the sequential nature of RNNs.
    \item \textbf{Scalability:} Transformers are highly scalable and capable of handling large input sequences without significantly dropping performance. This makes them ideal for source code analysis, where ASTs can vary widely in size and complexity.
\end{itemize}

% the problem 
Another issue is that most TBNN approaches tackle a classification problem for the source code but not regression tasks. Regression tasks such as source code performance prediction (predicting the execution time for the application prior to running it) can give the developer an early indication of the runtime behaviour of their source code. Samoaa et al.~\cite{SamoaaTEPGNN} indicate that trying the TNNs approaches for regression tasks will lead to poor efficiency compared to classification tasks.  That said, these solutions are not generic enough for any source code analysis tasks. We will use the benchmark models for source code analysis to prove this claim, leading to a high classification accuracy but in a regression context. Thus, we will use code2vec~\cite{Alon19}, TBCNN~\cite{CNN_tree}, and Transformer-based networks over AST(TBAST)~\cite{hua2022transformer} as the main benchmarks for regression tasks, taking into account that we have to make some changes in the architecture of these models to fit the regression tasks. 
% @Antonio add something more about GNN.
Additionally, we explore various GNN architectures, focusing on neighbourhood information sampling and aggregation within the AST, to further enrich our analysis framework.

 
% the approach
To address all the mentioned challenges, we develop our approach based on a cross-attention dual transformer, which utilizes sequences of source code tokens and AST nodes. By employing cross-attention mechanisms between the two transformers, our model aims to elucidate the influence of individual source code tokens on AST nodes, enhancing the understanding of code semantics. 

Through this study, we will answer the following question:
\begin{itemize}
    \item \textbf{Why does the TNN behave differently in regression tasks?}
\end{itemize}   

To that aim, we analyse the behaviour of each type of architecture (convolution, sequence, and GNN) for different levels of information: node level (for every node in the AST) as in TBCNN, GNNs, and sequential transformers or path level (a path in AST, which is a sequence of nodes) as in code2vec. 
% then we use these models to encode each path into a continuous vector as a representation, then the representations for paths will be pooled together to have the final vector that represents the entire AST. 
Since we have a regression value for each source code program, we have to map each AST to the regression value. Thus, the AST has to be represented as one vector. For that aim, we will aggregate the node and path representations through the models into one continuous vector. 
To increase the reliability, we use two different real-world datasets of performance measurements. The first dataset (\emph{OSSBuild}) is real build data collected from the continuous integration systems of four open-source systems. The second (\emph{HadoopTests}) is a larger dataset which we have collected ourselves by repeatedly executing unit tests from the Hadoop open-source system in a controlled environment. 
% the results 
The results show that our dual transformer approach Outperforms both TBNN and GNN-based approaches for both datasets.  
% The conclusion sentences. 
\textcolor{red}{Add the Contribution, which is a model-centric AI for employing both code tokens and trees in the transformer based on cross attentions. Datasets that can be used by the researchers in literature.  A framework that merges all TBNN with our own model so the researchers can use this open-source framework for different tasks. }


==> introduction.tex <==
% Introduction Revision
Deep learning has become pivotal in source code analysis, addressing a spectrum of tasks from classification and clone detection to bug identification and summarization~\cite{Bui2018,kanade2020,CNN_tree,Bui:21-2,Fang2020,Mehrotra2020,Hua2021,Li2021ICSE,Shi2021,Bui:21-1,Zhang:20,liu2021}. Traditionally, source code has been treated as plain text, relying on pattern matching and bag-of-words approaches, which neglect the rich semantic content inherent in the code~\cite{samoaaSLR2022,ALSABBAGH2022}. However, representing code as Abstract Syntax Trees (ASTs) offers a more nuanced view, capturing its syntactic structure and facilitating the application of tree-based neural networks (TNNs) like RvNN, TBCNN, and Tree-LSTM, which recursively compute node embeddings~\cite{AST_NN,DLCF,CNN_tree,SDF}.

Despite their advantages, deep learning models, particularly RNNs and CNNs, face significant limitations when applied to ASTs. RNNs, for instance, grapple with gradient vanishing, impeding their ability to learn from the deep structures of ASTs~\cite{mou2018tree}. CNNs, with their fixed-size windows, fail to capture the long-range dependencies within ASTs, crucial for understanding code semantics~\cite{mou2018tree}. Moreover, models that traverse ASTs from bottom to top can generate unwieldy sequential inputs, taxing computational resources and obscuring the syntactic architecture of ASTs~\cite{hua2022transformer}.

Acknowledging these challenges, our study pivots towards leveraging transformers as an alternative to traditional sequential models for source code analysis. Transformers excel in managing long dependencies through their self-attention mechanisms, enabling them to discern the intricate hierarchical relationships within ASTs. Their ability to process data in parallel enhances computational efficiency, a boon for handling ASTs' complexity. Moreover, the inherent flexibility of transformers allows them to adeptly capture both local and global context within the code structure, offering a more comprehensive understanding of code semantics than their RNN and CNN counterparts.

Given the limitations of TNNs in regression tasks and their predilection for classification, our research extends to exploring transformers in the context of source code performance prediction. This regression-focused approach aims to provide developers with early insights into their code's complexity, a facet not extensively covered by existing models~\cite{SamoaaTEPGNN}. We benchmark our study against established models like code2vec, TBCNN, and Transformer-based networks over AST (TBAST), adapting their architectures to suit regression tasks while also introducing our novel dual-transformer model tailored for this purpose. Additionally, we incorporate GNNs to leverage neighbourhood information in ASTs, enriching our comparative analysis.

Our investigation seeks to unravel the distinct behaviours of convolutional, sequential, and GNN structures across various information levels within ASTs. By mapping ASTs to regression values and aggregating node and path representations into a unified vector, we aim to provide a holistic view of source code performance. This study is underpinned by empirical analysis using two real-world datasets: OSSBuild and HadoopTests, encompassing data from continuous integration systems and controlled execution environments, respectively.

Preliminary results affirm the superiority of our dual-transformer model over traditional benchmarks and GNN approaches, marking a significant advancement in source code analysis. This study not only highlights the potential of transformers in navigating the complexities of ASTs but also sets the stage for their broader application in programming language processing, promising enhanced efficiency and deeper semantic insights.


==> tables_drafts.tex <==
% \begin{table}[h!]
%     \centering
%     \begin{tabular}{l|c|c}
%          & OssBuilds & Hadoop \\
%          \hline
%      GCN &  0.07  &  0.076\\
%      GAT &  0.070  &  0.06\\
%      GIN &  0.059  &  0.079\\
%      GraphSage & 0.06 &0.06 \\ \hline
%      Code2Vec & 5.09 & 0.03 \\
%      TreeCNN & 5.6 & 0.03 \\
%      Transformer-Based & 3.34 & 0.8
     
%     \end{tabular}
%     \caption{test MSE on trees for logarithmic scaling}
%     \label{tab:MSE}
% \end{table}


%\begin{table*}[ht]
%    \label{tab:errorlog}
%    \caption{Test MSE, MAE, and person correlation for both datasets trees}
%    \centering
%    \begin{tabular}{l|ccc|ccc}
%    & \multicolumn{3}{c|}{OssBuilds} & \multicolumn{3}{c}{Hadoop} \\
%         \cline{2-7}
%    & MSE & MAE & Cor. & MSE & MAE & Cor. \\
%    & $\downarrow$ & $\downarrow$ & $\uparrow$ & $\downarrow$ & $\downarrow$ & $\uparrow$ \\
%         \hline
%     GCN &  $0.07 \pm 0.02$  & $0.21 \pm 0.03$  & $0.65 \pm 0.04$ & $0.06 \pm 0.02$ & $0.21 \pm 0.03$  & $0.52 \pm 0.05$ \\
%     GAT &  $0.07 \pm 0.01$  & $0.23 \pm 0.02$  & $0.61  \pm 0.03$ & $0.09 \pm 0.01$ & $0.25 \pm 0.02$  & $ 0.38 \pm 0.07$\\
%     GIN &  $0.08 \pm 0.01$ & $0.21 \pm 0.01$ & $ 0.60 \pm 0.04$ & $ 0.06 \pm 0.003$ & $0.20 \pm 0.006$  & $ 0.50 \pm 0.04$\\
%     \textbf{GraphSage} & $0.06 \pm 0.01$ & $0.20 \pm 0.02$ & $0.68 \pm 0.02$& $ 0.06 \pm 0.01$ & $0.21 \pm 0.02$  & $ 0.52 \pm 0.03$\\
%     \hline
     % $ \pm $ & $ \pm $ & $ \pm $  & $ \pm $ & $ \pm $ & $ \pm $ \\
%     Code2Vec & $0.029 \pm 0.0034$ & $0.132 \pm 0.0089$ & $0.570 \pm 0.0127$  & $0.024 \pm 0.0011$ & $0.125 \pm 0.0042$ & $0.508 \pm 0.0253$ \\
%     TreeCNN & $0.029 \pm 0.0032$ & $0.136 \pm 0.0099$ & $0.517 \pm 0.0251$  & $0.021 \pm 0.0009$ & $0.114 \pm 0.0052$ & $0.568 \pm 0.0196$ \\
%     Transformer-Based (small) & $0.183 \pm 0.1120$ & $0.368 \pm 0.1323$ & $0.311 \pm 0.0912$  & $0.184 \pm 0.1538$ & $0.342 \pm 0.1667$ & $0.315 \pm 0.1036$ \\
%     Transformer-Based (large) & $0.666 \pm 0.3248$ & $0.646 \pm 0.1682$ & $0.239 \pm 0.1024$  & $0.188 \pm 0.0766$ & $0.343 \pm 0.0714$ & $0.238 \pm 0.1306$ \\
%     \hline
%     \textbf{Dual-Transformer (small)} & $0.017 \pm 0.0050$ & $0.099 \pm 0.0166$ & $0.808 \pm 0.0349$  & $0.021 \pm 0.0116$ & $0.110 \pm 0.0288$ & $0.707 \pm 0.0653$ \\
%     \textbf{Dual-Transformer (large)} & $\textbf{0.014} \pm 0.0023$ & $\textbf{0.088} \pm 0.0065$ & $\textbf{0.820} \pm 0.0194$  & $\textbf{0.017} \pm 0.0036$ & $\textbf{0.097} \pm 0.0101$ & $\textbf{0.729} \pm 0.0385$ \\
%     \hline
%    \end{tabular} 
%\end{table*}


% \begin{table}[h!]
%     \centering
%     \begin{tabular}{l|ccc|ccc}
%     & \multicolumn{3}{c|}{OssBuilds} & \multicolumn{3}{c}{Hadoop} \\
%          \cline{2-7}
%     & MSE & MAE & Cor. & MSE & MAE & Cor. \\
%     & $\downarrow$ & $\downarrow$ & $\uparrow$ & $\downarrow$ & $\downarrow$ & $\uparrow$ \\
%          \hline
%      GCN &  0.07  & 0.21  & 0.60 & 0.05 & 0.19  & 0.48 \\
%      GAT &  0.07  & 0.24  & 0.62 & 0.06 & 0.21  & 0.43\\
%      GIN &  0.07  &  0.20 & 0.61 & 0.08 & 0.22  & 0.43\\
%      GraphSage & 0.06 & 0.19 & 0.69 & 0.06 & 0.20  & 0.47\\
%      \hline
%      Code2Vec & 0.03 & 0.13& 0.59  & 0.04 & 0.15 & 0.50 \\
%      TreeCNN & 0.03 &0.15 & 0.54 & 0.03 & \textbf{0.13}  & 0.57 \\
%      Transformer-Based & 0.03 & 0.13 & 0.61 & 0.03 & 0.14 & 0.60 \\
%      \hline
%      \textbf{Dual-Transformer} & \textbf{0.02} & \textbf{0.09} & \textbf{0.79} & \textbf{0.03}  & 0.14& \textbf{0.70}  \\
%      \hline
%     \end{tabular}
%     \caption{Test MSE, MAE, and person correlation for both datasets trees}
%     \label{tab:errorlog}
% \end{table}



%\begin{table}[h!]
%    \centering
%    \begin{tabular}{l|cc|cc}
%         & \multicolumn{2}{c|}{MSE} & \multicolumn{2}{c}{MAE} \\
%         \cline{2-5}
%         & OssBuilds & Hadoop & OssBuilds & Hadoop \\
%         \hline
%     GCN &  0.07  &  0.05 & 0.21 & 0.19 \\
%     GAT &  0.07  &  0.06 & 0.24 & 0.21 \\
%     GIN &  0.07  &  0.08 & 0.20 & 0.22 \\
%     GraphSage & 0.06 & 0.06 & 0.19 & 0.20 \\
%     \hline
%     \textbf{Dual-Transformer} & \textbf{0.02} & \textbf{0.03} & \textbf{0.09} & 0.14 \\
%     \hline
%     Code2Vec & 0.03 & 0.04 & 0.13 & 0.15 \\
%     TreeCNN & 0.03 & 0.03 & 0.15 & \textbf{0.13} \\
%     Transformer-Based & 0.03 & 0.03 & 0.13 & 0.14 \\
%     \hline
%    \end{tabular}
%    \caption{Test MSE and MAE on trees}
%    \label{tab:errorlog}
%\end{table}


%\begin{table}[h!]
%    \centering
%    \begin{tabular}{l|c|c}
%         & OssBuilds & Hadoop \\
%         \hline
%     GCN &  0.60  &  0.48\\
%     GAT &  0.62  &  0.43\\
%     GIN &  0.61  &  0.43\\ 
%     GraphSage & 0.69 & 0.47 \\ 
%     \hline
%     \textbf{Dual-Transformer} & \textbf{0.79} & \textbf{0.70}  \\
%     \hline
%     Code2Vec & 0.59 & 0.50 \\
%     TreeCNN & 0.54 & 0.57 \\
%     Transformer-Based & 0.61 & 0.60 \\
%     \hline
%    \end{tabular}
%    \caption{pearson correlations on trees}
%    \label{tab:pealog}
%\end{table}

% \begin{table}[h!]
%     \centering
%     \begin{tabular}{l|cc|cc}
%          & \multicolumn{2}{c|}{MSE} & \multicolumn{2}{c}{MAE} \\
%          \cline{2-5}
%          & OssBuilds & Hadoop & OssBuilds & Hadoop \\
%          \hline
%      GCN &  0.07  &  0.076 & 0.0 & 0.0 \\
%      GAT &  0.070  &  0.06 & 0.0 & 0.0 \\
%      GIN &  0.059  &  0.079 & 0.0 & 0.0 \\
%      GraphSage & 0.06 & 0.06 & 0.0 & 0.0 \\
%      \hline
%      Code2Vec & 12356290.71 & 0.03 & 744.59 & 0.15 \\
%      TreeCNN & 12000455.65 & 0.031 & 600.64 & 0.14 \\
%      Transformer-Based & 10862164.85 & 0.03 & 947.007 & 0.14 \\
%     \end{tabular}
%     \caption{Test MSE and MAE on trees for MinMax scaling}
%     \label{tab:errorminmax}
% \end{table}


% \begin{table}[h!]
%     \centering
%     \begin{tabular}{l|c|c}
%          & OssBuilds & Hadoop \\
%          \hline
%      GCN &  0.60  &  0.386\\
%      GAT &  0.54  &  0.42\\
%      GIN &  0.61  &  0.42\\ 
%      GraphSage & 0.62 & 0.47 \\ 
%      \hline
%      Code2Vec & 0.0072 & 0.56 \\
%      TreeCNN & 0.09 & 0.54 \\
%      Transformer-Based & 0.63 & 0.60
%     \end{tabular}
%     \caption{pearson correlations on trees for MinMax scaling}
%     \label{tab:peaminmax}
% \end{table}
